What if we Increase the Number of Objectives? Theoretical and Empirical Implications for Many-objective Optimization

The difficulty of solving a multi-objective optimization problem is impacted by the number of objectives to be optimized. The presence of many objectives typically introduces a number of challenges that affect the choice/design of optimization algorithms. This paper investigates the drivers of these challenges from two angles: (i) the influence of the number of objectives on problem characteristics and (ii) the practical behavior of commonly used procedures and algorithms for coping with many objectives. In addition to reviewing various drivers, the paper makes theoretical contributions by quantifying some drivers and/or verifying these drivers empirically by carrying out experiments on multi-objective NK landscapes and other typical benchmarks. We then make use of our theoretical and empirical findings to derive practical recommendations to support algorithm design. Finally, we discuss remaining theoretical gaps and opportunities for future research in the area of multi- and many-objective optimization.

==> Comments_SpecialIssue.tex <==
Proposed structure: 
Section 1: 
\textbf{Christiane + All:} Standard introduction

Section 2. 
\textbf{Christiane + All:} Background section

Section 3: Theory I - Problem characteristics (current 2)

Section 4: Theory II - Algorithms (current 3)

Section 5. Case studies + experimental results

Section 6: Conclusion and future work


Possible Extensions (current version)
Section 2.1: 
\textbf{Richard+Christiane:} Do experiment for distance-based problems on how proportion of POS changes as nr of objectives increases. 

Section 2.3: 
\textbf{Arnaud+Richard+Christiane:} Verify equation of expected number of non-dominated solutions. Estimating the proportion of non-dominated solutions in random populations (Section 2.3) for test problems ==> This should be similar to Fig. 1 for ρMNK-landscapes, but this could be a nice way for us to have similar measures for (continuous) location problems by discretizing the space. 

Section 2.6: 
\textbf{Richard:} Expand section with text and potentially simple theoretical/experimental analysis of impact of many heterogeneous objectives on search. For example, is we assume that evaluation times per objective follow a normal distribution, then what is the effect on the total number of solutions that can be evaluated fully (i.e. on all objectives) within a fixed budget (time limit) → this would have practical implications. 

Section 3.1:
\textbf{Arnaud+ Andrzej:} Measuring the number of comparisons per objective (and maybe per solution as well, to show the difference) performed by archiving when the number of objectives grows. 
Link results and section to what was observed in 2020 paper by Jonathan entitled "Data Structures for Non-Dominated Sets: Implementations and
Empirical Assessment of Two Decades of Advances". 
Arnaud will generate datasets for 6, 8 and 9 objectives. Arnaud will also sorted data.  

Sections 3.1 + 3.2: 
\textbf{Andrzej: } I agree that considering other data structures than ND-Tree would be great as well. Look at alternative data structures to ND-Tree. Done. 

Sections 3.3:
Christiane: Start Section 3.3.1 with Generation Equation (1), then weighted sum, then Tschebyscheff, then (b), then e-constraints, and shorten (d) and (e). We can put material in Appendix if needed.  

Sections 3.3 and 3.4: 
\textbf{Still to be discussed: }Maybe address the question “On the  other  hand,  the question remains if the size of the confidence intervals should be reduced with growing number of objectives or growing mu.” by experimental analysis on test.Measuring the hypervolume approximation quality (exact vs Monte-Carlo sampling) w.r.t. the number of objectives, the approximation-set size and the number of sampling points.

Also relevant paper. 
\url{https://ore.exeter.ac.uk/repository/bitstream/handle/10871/36825/fieldsend_gecco_2019_hypervolume.pdf?sequence=1&isAllowed=y}


Note (RA): we have singled out hypervolume as a performance metric for MOO algorithms. Another popular metric is IGD, which I think we should put in context too. We should refer to this paper too https://iridia.ulb.ac.be/~leonardo/publications/conferences/BezLopStu2017.pdf

Determine switching points  (after how many objectives does Monte Carlo sampling become faster than exact computation) as a function of nr of points sampled and shape of Pareto front. 


Section 3.3:
\textbf{Still to be discussed: } Think if different scalarizing functions would show similar behaviour. 

Section 3.5: 
\textbf{Move section to Section 6 as doing all these experiments with different algorithms feels as too much work and not necessary: }Here we could demonstrate some of conclusions (e.g. impact of distances on coverage) using experiments run on (our and/or other) test problems. 

It was decided to compute distances between pair-wise randomly selected Pareto optimal solutions to confirm the theory that crossover becomes important as the problem scale increases (in terms of objectives) to bridge between distant hotpots of solutions. Distances will be computed in the objective and decision space starting with Euclidean distances (other distances may be considered later too).  

Section 4:  
\textbf{Move to Section 5: } We can discuss if and how the number of objectives (if we have many) affects the generation of test instances (be it an NK landscape instance, distance-based problem instance, or a location problem instance)


Next meeting Friday 15 May, 9am.  
